QuaSE: Accurate Text Style Transfer under Quantifiable Guidance

We propose the task of Quantifiable Sequence Editing (QuaSE): editing an input sequence to generate an output sequence that satisfies a given numerical outcome value measuring a certain property of the sequence, with the requirement of keeping the main content of the input sequence. For example, an input sequence could be a word sequence, such as review sentence and advertisement text. For a review sentence, the outcome could be the review rating; for an advertisement, the outcome could be the click-through rate. The major challenge in performing QuaSE is how to perceive the outcome-related wordings, and only edit them to change the outcome. In this paper, the proposed framework contains two latent factors, namely, outcome factor and content factor, disentangled from the input sentence to allow convenient editing to change the outcome and keep the content. Our framework explores the pseudo-parallel sentences by modeling their content similarity and outcome differences to enable a better disentanglement of the latent factors, which allows generating an output to better satisfy the desired outcome and keep the content. The dual reconstruction structure further enhances the capability of generating expected output by exploiting the couplings of latent factors of pseudo-parallel sentences. For evaluation, we prepared a dataset of Yelp review sentences with the ratings as outcome. Extensive experimental results are reported and discussed to elaborate the peculiarities of our framework.

==> graphvizzz.tex <==
% graphvizzz.sty
% Ives van der Flaas
% ives.vdf@gmail.com
% http://code.google.com/p/graphvizzz/
%
% Based on graphviz.sty by Mark Aufflick 2006-03-25
% Based on graphviz.tex by Derek Rayside 2003

% add the following lines to your preamble:

% \usepackage[pdftex]{graphicx}
% \usepackage{graphvizzz}

% parameters to \digraph:
% 1 - parameters for \includegraphics (optional; default value is "scale=1")
% 2 - name of the digraph
% 3 - body of the digraph

\ProvidesPackage{graphvizzz}


\newcommand{\digraph}[3][scale=1]{ 
  \newwrite\dotfile 
  \immediate\openout\dotfile=#2.dot 
  \immediate\write\dotfile{digraph #2 {\string#3}} 
  \immediate\closeout\dotfile
  \immediate\write18{dot -Tpdf #2.dot > #2.pdf}
  \IfFileExists{#2.pdf}
  % the pdf exists: include it 
  { \includegraphics[#1]{#2} } 
  % the pdf was not created - show a hint
  {   
      The PDF file displaying your dot graph could not be created. 
      This usually means one of
      two things:
        \begin{itemize}
        \item dot is not in your path
        \item write18 is not enabled
        \end{itemize}
        Please check http://code.google.com/p/graphvizzz/ for more
        information. 
      
  } 
}

\newcommand{\graph}[3][scale=1]{ 
  \newwrite\dotfile 
  \immediate\openout\dotfile=#2.dot 
  \immediate\write\dotfile{graph #2 {\string#3}} 
  \immediate\closeout\dotfile
  \immediate\write18{dot -Tpdf #2.dot > #2.pdf}
  \IfFileExists{#2.pdf}
  % the pdf exists: include it 
  { \includegraphics[#1]{#2} } 
  % the pdf was not created - show a hint
  {   
      The PDF file displaying your dot graph could not be created. 
      This usually means one of
      two things:
        \begin{itemize}
        \item dot is not in your path
        \item write18 is not enabled
        \end{itemize}
        Please check http://code.google.com/p/graphvizzz/ for more
        information. 
      
  } 
}


==> model.tex <==
% \usepackage{mathtools} 
\begin{tikzpicture}

    \node[obs]  (r) {$R$};
    \node[latent, below = 0.75of r] (y){$Y$};
    \node[obs, below = 0.75of y] (x) {$X$};
    \node[latent, below = 0.75of x] (z) {$Z$};
	
	\edge[left = 30]{y}{r};
	\edge[bend left = 30]{y}{x};
	\edge[bend left = 30]{x}{y};
	\edge[bend left = 30]{x}{z};
	\edge[bend left = 30]{z}{x};
    
    
    
    \node[latent, right = 2of y, yshift = 1 cm] (Y){$y$};
    \node[obs, below = of Y] (X) {$x$};
    \node[latent, below = of X] (Z) {$z$};
	
%	\edge[left = 30]{Y}{R};
%	\edge[bend left = 30]{Y}{X};
	\edge[left = 30]{X}{Y};
	\edge[left = 30]{X}{Z};
%	\edge[bend left = 30]{Z}{X};
	
%	\node[obs ,right = 4 of R]  (R2) {$r'$};
    \node[latent, right = 5 of Y] (Y2){$y'$};
    \node[obs, below = of Y2] (X2) {$x'$};
    \node[latent, below = of X2] (Z2) {$z'$};
	
%	\edge[left = 30]{Y2}{R2};
%	\edge[bend left = 30]{Y2}{X2};
	\edge[left = 30]{X2}{Y2};
	\edge[left = 30]{X2}{Z2};
%	\edge[bend left = 30]{Z2}{X2};
	
	\node[draw = none, fill = none,  right = 1.7of X] (Dxx){$f(x,x')$};
	\node[draw = none, fill= none, right = 1.7of Y,yshift = 0.5 cm] (Dyy) {$h(y,y')$};
	\node[draw = none, fill = none, below = 0.2of y, xshift = -0.7 cm]{$E_1$};
	\node[draw = none, fill = none, below = 0.2of y, xshift = 0.7 cm]{$D$};
	\node[draw = none, fill = none, below = 0.2of r, xshift = -0.25 cm]{$F$};
	\node[draw = none, fill = none, below = 0.2of x, xshift = -0.7 cm]{$D$};
	\node[draw = none, fill = none, below = 0.2of x, xshift = 0.7 cm]{$E_2$};
	\node[draw = none, fill = none, below = 0.2of Y, xshift = 0.25 cm]{$E_1$};
	\node[draw = none, fill = none, below = 0.2of Y2, xshift = -0.25 cm]{$E_1$};
	\node[draw = none, fill = none, below = 0.2of X2, xshift = -0.25 cm]{$E_2$};
	\node[draw = none, fill = none, below = 0.2of X, xshift = 0.25 cm]{$E_2$};
	
	\node[draw,fill=none, below =0.5of Dxx] (Discrim){$\mathcal L_{d-rec}$};
	\node[draw, fill=none, below =0.5of Discrim] (Min){$\mathcal L_{sim}$};
	\node[draw , fill = none, below = 0.5of Dyy] (Reg){$\mathcal L_{diff}$};
	
	
	\drawdotted {Dxx} {Reg};
	\drawdotted {Dyy} {Reg};
	\drawdotted {X} {Discrim};
	\drawdotted {X2} {Discrim};
	\drawdotted {Z}{Min};
	\drawdotted {Z2}{Min};
	
	\edge {X,X2}{Dxx};
	\edge {Y,Y2}{Dyy};
	%\edge {Dxx}{Dyy};
	
\end{tikzpicture}

==> name_old.tex <==
% \usepackage{mathtools} 
\begin{tikzpicture}
    \node[obs]  (R) {$R(r)$};
    \node[latent, below = of R] (Y){$Y(y)$};
    \node[obs, below = 2of Y] (X) {$X(x)$};
    \node[latent, below = 2of X] (Z) {$Z(z)$};
	
	\edge[left = 30]{Y}{R};
	\edge[bend left = 30]{Y}{X};
	\edge[bend left = 30]{X}{Y};
	\edge[bend left = 30]{X}{Z};
	\edge[bend left = 30]{Z}{X};
	
	\node[obs ,right = 4 of R]  (R2) {$r'$};
    \node[latent, below =1.1 of R2] (Y2){$y'$};
    \node[obs, below = 2.2of Y2] (X2) {$x'$};
    \node[latent, below = 2.2of X2] (Z2) {$z'$};
	
	\edge[left = 30]{Y2}{R2};
	\edge[bend left = 30]{Y2}{X2};
	\edge[bend left = 30]{X2}{Y2};
	\edge[bend left = 30]{X2}{Z2};
	\edge[bend left = 30]{Z2}{X2};
	
	\node[draw = none, fill = none,  right = of X] (Dxx){$diff(x,x')$};
	\node[draw = none, fill= none, right = of Y] (Dyy) {$diff(y,y')$};
	
	\node[draw,fill=none, below =0.75of Dxx] (Discrim){$\mathcal L_{d-vae}$};
	\node[draw, fill=none, below =of Discrim] (Min){$\mathcal L_{min}$};
	\node[draw , fill = none, below = 0.75of Dyy] (Reg){$\mathcal L_{diff}$};
	
	\drawdotted {Dxx} {Reg};
	\drawdotted {Dyy} {Reg};
	\drawdotted {X} {Discrim};
	\drawdotted {X2} {Discrim};
	\drawdotted {Z}{Min};
	\drawdotted {Z2}{Min};
	
	\edge {X,X2}{Dxx};
	\edge {Y,Y2}{Dyy};
	%\edge {Dxx}{Dyy};
	
\end{tikzpicture}

==> notation_table.tex <==
\small
    \centering
    \begin{tabular}{c|l}
    \hline
         $X$& A sentence represented by a sequence of words \\
         $R$& The outcome associated with the sentence $X$\\
         $Y$& The outcome factor disentangled from the sentence $X$\\
         $Z$& The content factor disentangled from the sentence $X$\\ \hline
         $(x,x')$ & A pair of pseudo-parallel sentences with similar contents but different outcomes\\
         $diff(x,x')$& The explicit wording difference between $x$ and $x'$, defined in Equation \ref{diff} \\
         $diff(y,y')$& The difference between the outcome factors $y$ and $y'$, defined in Equation \ref{diff}\\ \hline
         $E_1$ & The encoder that generates the outcome factor from the sentence $X$\\
         $E_2$ &  The encoder that generates the content factor from the sentence $X$\\
         $D$ &  The decoder that generates a sentence from an outcome factor $Y$ and a content factor $Z$\\
         $F$ & The fully connected network that projects the outcome factor $Y$ to the outcome $R$\\
         $U$ & The fully connected network that aligns $diff(x,x')$ with $diff(y,y')$ \\ \hline 
         $\mathcal L_{rec}$ & The reconstruction loss between a sentences and its reconstructed sentence \\ 
         $\mathcal L_{kl}$ & The KL-divergence between the variation posterior distribution and the prior\\ 
         $\mathcal L_{mse}$ & The prediction loss of $F$\\ 
         $\mathcal L_{diff}$ & The regression loss of $U$\\
         $\mathcal L_{sim}$ & The minimization loss between $z$ and $z'$\\
         $\mathcal L_{d-rec}$ & The dual reconstruction loss between $x$ and $x'$ \\ \hline
    \end{tabular}
    \caption{Notations in the model.}
    \label{notions}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
%\tikzstyle{dashplate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node

\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

\newcommand{\drawdotted}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      %\path (\x) edge [->,#1] (\y) ;%
      \draw[dotted,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


